Knowledge Transfer by Discriminative Pre-training for Academic Performance Prediction

The needs for precisely estimating a student's academic performance have been emphasized with an increasing amount of attention paid to Intelligent Tutoring System (ITS). However, since labels for academic performance, such as test scores, are collected from outside of ITS, obtaining the labels is costly, leading to label-scarcity problem which brings challenge in taking machine learning approaches for academic performance prediction. To this end, inspired by the recent advancement of pre-training method in natural language processing community, we propose DPA, a transfer learning framework with Discriminative Pre-training tasks for Academic performance prediction. DPA pre-trains two models, a generator and a discriminator, and fine-tunes the discriminator on academic performance prediction. In DPA's pre-training phase, a sequence of interactions where some tokens are masked is provided to the generator which is trained to reconstruct the original sequence. Then, the discriminator takes an interaction sequence where the masked tokens are replaced by the generator's outputs, and is trained to predict the originalities of all tokens in the sequence. Compared to the previous state-of-the-art generative pre-training method, DPA is more sample efficient, leading to fast convergence to lower academic performance prediction error. We conduct extensive experimental studies on a real-world dataset obtained from a multi-platform ITS application and show that DPA outperforms the previous state-of-the-art generative pre-training method with a reduction of 4.05% in mean absolute error and more robust to increased label-scarcity.

==> related_works.tex <==
\section{Related Works}
\subsection{Transfer Learning}
Transfer learning is a widely studied research topic across different domains of machine learning.
A commonly taken approach in NLP field is pre-training a model on a large corpus and fine-tuning the pre-trained model on downstream tasks, such as machine translation, question answering, and reading comprehension.
\cite{radford2018improving,radford2019language,brown2020language} made dramatic improvements in several downstream tasks by pre-training a model with an autoregressive language modeling objective.
The further progress was made with other pre-training objectives including masked language modeling \cite{devlin2018bert}, permutation language modeling \cite{yang2019xlnet}, and discriminative pre-training \cite{clark2020electra}.
In computer vision domain, \cite{chen2020generative} and \cite{dosovitskiy2020image} outperformed the previous approaches by pre-training a model in pixel-wise and patch-wise fashion, respectively.

Transfer learning has also been applied to a large body of work for AIEd tasks.
\cite{su2018exercise,liu2019ekt}, \cite{sung2019improving}, and \cite{huang2017question} computed latent representations of exercises or students’ answers by mapping words in their text descriptions to embedding vectors pre-trained from a large corpus for Knowledge Tracing, answer grading, and exercise difficulty prediction, respectively.
\cite{ding2019transfer} introduced Auto-Encoder (AE)-based transfer learning method for course dropout prediction in edX Massive Open Online Course (MOOC) platform.
They proposed two different transfer learning methods, passive AE transfer and active AE transfer, and investigated transferability across similar and dissimilar MOOC courses.

\subsection{Student Performance Prediction}
Given records of learning activities of a student, estimating their grade, score, other academic status, such as pass/fail, on a specific course, or eligibility of graduation is an important task for many downstream educational applications.
Student performance prediction has many similarities with Knowledge Tracing \cite{corbett1994knowledge,piech2015deep,zhang2017dynamic,choi2020towards,shin2020saint+} which commonly formulated as a task of sequentially predicting a student's response correctness to the next given exercise.
However, in this subsection, we make a distinction between student performance prediction and Knowledge Tracing by narrowing down the range of student performance prediction to tasks where a prediction label is only given at the end of the learning activities sequence, and focus on the previous studies that meet this condition.

Wide range of approaches for student performance prediction have been proposed including Matrix Factorization (MF) \cite{ren2017grade,zhong2019constrained}, MLP \cite{raga2019early}, RNN \cite{kim2018gritnet,hu2019reliable,li2020student}, and Graph Neural Network (GNN) \cite{hu2019academic,karimi2020online,li2020peer}.
\cite{ren2017grade} proposed integrating course-wise influence effects and temporal effects in the MF algorithm for predicting grades that a student will get from courses in the next term.
Similar to other MF-based methods, the competence that a student has over a course was calculated by dot product between latent vectors of the student and the course.
However, the terms representing the student’s previous performance over other courses were added to the objective function, which allows to model pairwise course relationships.
\cite{zhong2019constrained} observed that some courses are very popular, while some are not, resulting in unbalanced distribution of course selection rate. To reduce the influence of course selection rate, additional terms were integrated into the MF objective function to force predicted scores approach toward course average scores.

With the rise of deep learning, several studies explored student performance prediction problem from a deep learning perspective, and adopted Neural Networks (NN) as a basic building block for their proposed model.
\cite{raga2019early} developed MLP model that predicts pass/fail of several classes based on online learning activity logs collected from the Moodle Learning Management System.
\cite{kim2018gritnet} proposed BiLSTM-based graduation prediction model which outperformed logistic regression-based baseline model on the Udacity dataset.
\cite{li2020student} suggested Sequential Prediction based on Deep Network (SPDN) model which is a combination of Multi-source Fusion Convolutional Neural Network (MFCNN) and BiLSTM.
The MFCNN component in the SPDN model computed compressed representation of a student’s multiple learning activities in weeks. The representation was then fed to the BiLSTM to estimate the student’s at-risk probability.
Not only the prediction accuracy, reliability and interpretability of predictions are also important considerations for many educational systems.
\cite{hu2019reliable} estimated uncertainties of MLP and LSTM models’ grade predictions through MC-dropout \cite{gal2016dropout} technique and computed the influence of a prior course grade on a target course grade to provide explainability to the models’ predictions.

Recently, with the consideration of course dependency structure, GNN-based models have become emerging approaches for student performance prediction.
Deep Online Performance Evaluation framework introduced in \cite{karimi2020online} learned student and course embeddings through relational GNN from student course relations knowledge graph.
\cite{hu2019academic} incorporated the attention layer into the Graph Convolutional Network to help identify prior courses important for predictions.
\cite{li2020peer} constructed a student-interaction-exercise graph and presented Residual Relational GNN which incorporated residual connections between different convolutional layers and original features.

\subsection{Transfer Learning for Student Performance Prediction}
Like other domains in machine learning, transfer learning has also been successfully applied to student performance prediction.
Sparse AE-based pre-training approach for grade prediction was proposed in \cite{guo2015predicting} where each hidden layer in NN was greedily pre-trained in unsupervised fashion.
\cite{hunt2017transfer} employed TrAdaBoost \cite{10.1145/1273496.1273521} algorithm, an extended version of the AdaBoost algorithm for transfer learning, for graduation prediction.
QuesNet \cite{yin2019quesnet} is an exercise embedding model pre-trained with heterogeneous contents in an exercise including text, images and side information, such as required knowledge to solve the exercise.
The authors suggested two pre-training objectives: Holed Language Modeling (HLM) and Domain-Oriented Objective (DOO).
The HLM aimed to learn low level representation and the objective of DOO was to capture domain specific logic and knowledge.
\cite{choi2020assessment} introduced Assessment Modeling, a pre-training framework for label-scarce educational problems.
They pre-trained a model to predict assessments, interactive features with pedagogical meaning, and fine-tuned the model appropriate for several label-scarce educational tasks including exam score prediction and review correctness prediction.


